A Dynamical Systems Approach for Static Evaluation in Go

In the paper arguments are given why the concept of static evaluation has the potential to be a useful extension to Monte Carlo tree search. A new concept of modeling static evaluation through a dynamical system is introduced and strengths and weaknesses are discussed. The general suitability of this approach is demonstrated.

==> Makefile <==
# diago package: 
#	DIAgrams for GO, by Thomas Wolf
#	04.2007

TEXMF=/usr/share/texmf

FILES = ${TEXMF}/tex/latex/misc/diago.sty \
	${TEXMF}/tex/latex/misc/Ugoss.fd \
	${TEXMF}/metafont/misc/godig.mf \
	${TEXMF}/metafont/misc/gostone.mf \
	${TEXMF}/metafont/misc/goss10.mf \
	${TEXMF}/fonts/tfm/public/misc/goss10.tfm

all:
	@echo " "
	@echo " diago: please use one of the following:"
	@echo " "
	@echo "  make install	- install (need to be root)"
	@echo "  make remove	- remove a previous installation (need to be root)"
	@echo "  make tar	- make a ../diago.tgz file, ready for distribution"
	@echo " "

tar:
	cd ../ ; tar -zcf diago.tgz diago/diago.sty diago/Ugoss.fd \
	diago/godig.mf diago/gostone.mf diago/goss10.mf diago/goss10.tfm \
	diago/Makefile diago/test.tex diago/readme
	@echo " "
	@echo " ../diago.tgz ready for distribution"
	@echo " "

install:
	@install -D -m 644 diago.sty	${TEXMF}/tex/latex/misc/diago.sty
	@install -D -m 644 Ugoss.fd	${TEXMF}/tex/latex/misc/Ugoss.fd
	@install -D -m 644 godig.mf	${TEXMF}/metafont/misc/godig.mf
	@install -D -m 644 gostone.mf	${TEXMF}/metafont/misc/gostone.mf
	@install -D -m 644 goss10.mf	${TEXMF}/metafont/misc/goss10.mf
	@install -D -m 644 goss10.tfm	${TEXMF}/fonts/tfm/public/misc/goss10.tfm
	@echo " "
	@echo " diago files installed"
	@echo " "
	/usr/bin/texhash
	@echo " "
	@echo " tex ls-lR rehashed"
	@echo " "

remove:
	rm -f ../diago.tgz ${FILES}
	@echo " "
	@echo " diago files removed"
	@echo " "



==> diago/Makefile <==
# diago package: 
#	DIAgrams for GO, by Thomas Wolf
#	04.2007

TEXMF=/usr/share/texmf

FILES = ${TEXMF}/tex/latex/misc/diago.sty \
	${TEXMF}/tex/latex/misc/Ugoss.fd \
	${TEXMF}/metafont/misc/godig.mf \
	${TEXMF}/metafont/misc/gostone.mf \
	${TEXMF}/metafont/misc/goss10.mf \
	${TEXMF}/fonts/tfm/public/misc/goss10.tfm

all:
	@echo " "
	@echo " diago: please use one of the following:"
	@echo " "
	@echo "  make install	- install (need to be root)"
	@echo "  make remove	- remove a previous installation (need to be root)"
	@echo "  make tar	- make a ../diago.tgz file, ready for distribution"
	@echo " "

tar:
	cd ../ ; tar -zcf diago.tgz diago/diago.sty diago/Ugoss.fd \
	diago/godig.mf diago/gostone.mf diago/goss10.mf diago/goss10.tfm \
	diago/Makefile diago/test.tex diago/readme
	@echo " "
	@echo " ../diago.tgz ready for distribution"
	@echo " "

install:
	@install -D -m 644 diago.sty	${TEXMF}/tex/latex/misc/diago.sty
	@install -D -m 644 Ugoss.fd	${TEXMF}/tex/latex/misc/Ugoss.fd
	@install -D -m 644 godig.mf	${TEXMF}/metafont/misc/godig.mf
	@install -D -m 644 gostone.mf	${TEXMF}/metafont/misc/gostone.mf
	@install -D -m 644 goss10.mf	${TEXMF}/metafont/misc/goss10.mf
	@install -D -m 644 goss10.tfm	${TEXMF}/fonts/tfm/public/misc/goss10.tfm
	@echo " "
	@echo " diago files installed"
	@echo " "
	/usr/bin/texhash
	@echo " "
	@echo " tex ls-lR rehashed"
	@echo " "

remove:
	rm -f ../diago.tgz ${FILES}
	@echo " "
	@echo " diago files removed"
	@echo " "


